Robust Model Predictive Control with Polytopic Model Uncertainty through System Level Synthesis

We propose a robust model predictive control (MPC) method for discrete-time linear systems with polytopic model uncertainty and additive disturbances. Optimizing over linear time-varying (LTV) state feedback controllers has been successfully used for robust MPC when only additive disturbances are present. However, it is challenging to design LTV state feedback controllers in the face of model uncertainty whose effects are difficult to bound. To address this issue, we propose a novel approach to over-approximate the effects of both model uncertainty and additive disturbances by a filtered additive disturbance signal. Using the System Level Synthesis framework, we jointly search for robust LTV state feedback controllers and the bounds on the effects of uncertainty online, which allows us to reduce the conservatism and minimize an upper bound on the worst-case cost in robust MPC. We provide a comprehensive numerical comparison of our method and representative robust MPC methods from the literature. Numerical examples demonstrate that our proposed method can significantly reduce the conservatism over a wide range of uncertainty parameters with comparable computational effort as the baseline methods.

==> closed_loop.tex <==
% closed-loop properties
\label{sec:closed_loop}
In this section, we discuss the closed-loop properties of SLS MPC. In practice, we want the closed-loop trajectories to (a) satisfy all constraints robustly, and (b) converge to the origin when the uncertainty diminishes.  The former property is captured by the notion of recursive feasibility, and the latter by the input-to-state stability (ISS)~\citep{jiang2001input}. Next, we discuss the challenges of providing recursive feasibility guarantees for SLS MPC through the standard shifting arguments~\citep[Chapter 12]{borrelli2017predictive}, and use the shrinking horizon strategy proposed in~\citep{bujarbaruah2022robust} as a solution. 

\subsection{Terminal set construction}
To provide closed-loop guarantees for MPC, we assume a robustly stabilizing local linear state-feedback controller is available and choose its induced robust forward invariant set as the terminal set $\mathcal{X}_T$. Such assumption is common in the robust MPC literature~\citep{kothare1996robust, langson2004robust, fleming2014robust, bujarbaruah2022robust}. 

\begin{assumption} \label{assump:robust_stable}
	A linear state feedback controller $\kappa(x) = Kx$ is known such that the $\hat{A} + \Delta_A + (\hat{B} + \Delta_B) K$ is stable for all $(\Delta_A, \Delta_B) \in \mathcal{P}$.
\end{assumption}

\begin{assumption} \label{assump:robust_invariant}
	The terminal set $\mathcal{X}_T$ is a robust forward invariant set under the local controller $\kappa(x) = Kx$, i.e., for all $x \in \mathcal{X}_T$, we have $x \in \mathcal{X}, Kx \in \mathcal{U}$, and $((\hat{A} + \Delta_A) + (\hat{B} + \Delta_B) K)x + w \in \mathcal{X}_T$ for all $(\Delta_A, \Delta_B) \in \mathcal{P}, w \in \mathcal{W}$.
\end{assumption}

The local controller $\kappa(x)$ can be synthesized by solving a semidefinite program~\citep{boyd1994linear, kothare1996robust}, and the terminal set can be found using an iterative algorithm~\citep{pluymers2005efficient}. However, they are not sufficient to guarantee recursive feasibility of SLS MPC with a fixed horizon $T$, i.e., Problem~\eqref{eq:convex_inner_approx} is feasible for all time steps with the initial condition as the closed-loop state $x(k)$. The main challenge is elaborated below. 

\textbf{Challenge of proving recursive feasibility}: The standard proof of recursive feasibility utilizes a shifting argument~\citep[Chapter 12]{borrelli2017predictive} that constructs a feasible solution to the robust OCP at $x(k+1)$ by attaching the local controller $\kappa(x)$ from Assumption~\ref{assump:robust_stable} to the control policies synthesized at $x(k)$. For example, assume at $x(k)$ a feasible solution of the robust OCP~\eqref{eq:robustOCP} generates a sequence of robust policies 
\begin{equation*}\label{eq:robust_policy_k}
	U_k = \{ u_{k\vert k}^*, u_{k+1\vert k}^*(\cdot), \cdots, u_{k+T_k-1 \vert k}^*(\cdot)  \}
\end{equation*}
where $u_{k \mid k}^*$ is applied to drive the system to $x(k+1)$ and $u_{t \mid k}(\cdot)$ denotes the predicted feedback policy at time $t$. Then, the shifting argument aims to show that the following candidate solution
\begin{equation*}
	U_{k+1} = \{ u_{k+1\vert k}^*(\cdot), \cdots, u_{k+T_k-1 \vert k}^*(\cdot),\kappa(\cdot) \}
\end{equation*}
is feasible to the robust OCP with initial condition $x(k+1)$, which proves recursive feasibility of MPC. 

However, such argument cannot be applied to SLS MPC. In Problem~\eqref{eq:convex_inner_approx}, the over-approximation of the uncertainty effects is derived in the space of system responses and used to tighten the constraints. While we can conveniently construct the candidate solution $U_{k+1}$ in the controller space, showing that the system responses induced by $U_{k+1}$ satisfy all the tightened constraints in~\eqref{eq:convex_inner_approx} with $x(k+1)$ as the initial condition remains an open problem. This issue is also encountered in~\citep{bujarbaruah2022robust} which considers LTV state feedback controller design. To guarantee robust constraint satisfaction at all time steps and ISS of the closed-loop system, we equip SLS MPC with  the shrinking horizon strategy proposed in~\citep{bujarbaruah2022robust} which is stated below. 

\subsection{Shrinking horizon and closed-loop guarantees}
We assume at time $k=0$, Problem~\eqref{eq:convex_inner_approx} is feasible with horizon $T$, generating policies (state feedback controllers)
\begin{equation}\label{eq:backup_policy}
	U_0 = \{ u_{0\vert 0}^*, u_{1\vert 0}^*(\cdot), \cdots, u_{T \vert 0}^*(\cdot)  \}
\end{equation}
that drive the system to the terminal set $\mathcal{X}_T$ in $T$ steps. We treat $U_0$ as a safe backup policy. Let $T_k$ denote the horizon of the robust OCP~\eqref{eq:convex_inner_approx} solved at time $k$ in SLS MPC. The following shrinking horizon strategy is applied
\begin{equation} 
	T_k = \begin{cases}
		T - k, & \textrm{if } k \in \{0, 1, \cdots, T-2\}, \\
		1, & \textrm{otherwise.}
	\end{cases}
\end{equation}
Additionally, we require that (i) when $T_k = 1$, instead of solving the tightened problem~\eqref{eq:convex_inner_approx}, we solve the robust OCP~\eqref{eq:robustOCP} exactly by enumerating all vertices of $(\Delta_A, \Delta_B)$ and $w_0$; (ii) when Problem~\eqref{eq:convex_inner_approx} with $T_k >1$ is infeasible, we apply the backup policy from $U_0$. Measures (i) and (ii) guarantee that the closed-loop trajectory reaches the terminal set $\mathcal{X}_T$ in at most $T$ steps and remains inside $\mathcal{X}_T$ thereafter. Under Assumption~\ref{assump:robust_invariant}, the robust OCP~\eqref{eq:robustOCP} with $T_k = 1$ is always feasible for $x(k) \in \mathcal{X}_T$. This naturally guarantees that the closed-loop trajectory satisfies all constraints robustly. Since for $k \geq T$, we solve the robust OCP~\eqref{eq:robustOCP} exactly with $T_k =1$ instead of Problem~\eqref{eq:convex_inner_approx}, the proof of ISS of the closed-loop system follows exactly from~\citep[Theorem 2]{bujarbaruah2022robust}.

%\begin{assumption} \label{assump:cost}
%When $T_k  = 1$, the cost function of the robust OCP~\eqref{eq:robustOCP} is given by $x_0^\top Q x_0 + u_0^\top R u_0 + x_1^\top P x_1$ such that $Q \succ 0, R \succ 0$, and $P \succ 0$ satisfies 
%\begin{equation*}
%x^\top (-P + (Q + K^\top R K) + \hat{A}_{cl}^\top P \hat{A}_{cl}) x \leq 0
%\end{equation*} 
%for all $x \in \mathcal{X}_T$ where $\hat{A}_{cl} = \hat{A} + \hat{B}K$. 
%\end{assumption}
%
%\begin{lemma}
%Let Assumption~\ref{assump:robust_stable} to~\ref{assump:cost} hold. With the shrinking horizon strategy, the closed-loop system is ISS. 
%\end{lemma}



==> defs.tex <==
% Environments
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}    
\newtheorem{remarks}{Remarks}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}    
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}    
%\newtheorem{proof*}{Proof}    
\newtheorem{proof}{Proof}
\newtheorem{assumption}{Assumption}    
\newtheorem{definition}{Definition}    
\newtheorem{problem}{Problem}    


% Sets of numbers
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}

% Vectors
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\xbar}{\bar{\x}}
\newcommand{\be}{\mathbf{e}}

% Optimization operators/notation
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\minimize}{minimize \quad}
\DeclareMathOperator*{\maximize}{maximize \quad}
\DeclareMathOperator*{\st}{subject\,\, to \quad}

% Functions
\newcommand{\norm}[1]{\left|\left| #1 \right|\right|}

% Operators
\newcommand{\id}{\text{Id}}
\newcommand{\prox}{\text{prox}}

\newcommand{\specialcell}[2][c]{%
	\begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}


